IterIS: Iterative Inference-Solving Alignment for LoRA Merging

Low-rank adaptations (LoRA) are widely used to fine-tune large models across various domains for specific downstream tasks. While task-specific LoRAs are often available, concerns about data privacy and intellectual property can restrict access to training data, limiting the acquisition of a multi-task model through gradient-based training. In response, LoRA merging presents an effective solution by combining multiple LoRAs into a unified adapter while maintaining data privacy. Prior works on LoRA merging primarily frame it as an optimization problem, yet these approaches face several limitations, including the rough assumption about input features utilized in optimization, massive sample requirements, and the unbalanced optimization objective. These limitations can significantly degrade performance. To address these, we propose a novel optimization-based method, named IterIS: 1) We formulate LoRA merging as an advanced optimization problem to mitigate the rough assumption. Additionally, we employ an iterative inference-solving framework in our algorithm. It can progressively refine the optimization objective for improved performance. 2) We introduce an efficient regularization term to reduce the need for massive sample requirements (requiring only 1-5% of the unlabeled samples compared to prior methods). 3) We utilize adaptive weights in the optimization objective to mitigate potential unbalances in LoRA merging process. Our method demonstrates significant improvements over multiple baselines and state-of-the-art methods in composing tasks for text-to-image diffusion, vision-language models, and large language models. Furthermore, our layer-wise algorithm can achieve convergence with minimal steps, ensuring efficiency in both memory and computation.

==> sec/X_suppl_solo.tex <==
\clearpage
\appendix % 标记开始附录
\renewcommand{\thesection}{\Alph{section}} 
\setcounter{page}{1}
\setcounter{equation}{8}
\setcounter{figure}{6}
\setcounter{table}{3}
\maketitlesupplementary
\noindent{In the supplementary materials, we provide:}
\begin{itemize}
\item  \textbf{Mathematical Proofs} (Section~\ref{sec:A}):  
   We present the mathematical proofs for the equations and properties of our proposed algorithm, as discussed in the main text.
\item \textbf{Datasets and Experimental Setup} (Section~\ref{sec:B}):  
   This section details the datasets employed in our experiments, the LoRA training configuration, and the key settings of the baseline implementations.
\item  \textbf{Ablation Studies} (Section~\ref{sec:C}):  
   We report the results of ablation studies, demonstrating the necessity of the three mechanisms integrated into our algorithm.
\item \textbf{Experimental Results} (Section~\ref{sec:D}):  
   A detailed presentation of the experimental results is provided in this section.
\item \textbf{Workflow and Analysis} (Section~\ref{sec:E}):  
   Finally, we illustrate the complete workflow of IterIS and conduct an analysis of the efficiency and limitations of our approach.
\end{itemize}
\section{Detailed Mathematical Derivation}
\label{sec:A}
\subsection{Linear Merging}
\label{sec:linear_merging_subsec}
Consider the following optimization problem:
% \begin{equation}
%     W^{*} = \mathop{\arg\min}_{W} E \left[\sum_{i=1}^N \lambda_i \| W_i^{T} x_i - W^{T} x_i \|_{F}^2 \right]
%     \label{eq:linear_app}
% \end{equation}
\begin{equation}
\small
    \bm{{W}^{*}} = \mathop{\arg\min}_{\bm{W}} \mathbb{E}_{\mathcal{\bm{X}}} [ \sum_{i=1}^{N} \lambda_i \| \bm{W}_i^{T} {\bm{\mathcal{X}}_i} - \bm{{W}^{T}} {\bm{\mathcal{X}}_i} \|_F^2 ]
    \label{eq:linear}
\end{equation}
where \( \mathbb{E}_\mathcal{\bm{X}}[\cdot] \) denotes the expectation with respect to \( \mathcal{\bm{X}} \) ( \( \mathcal{\bm{X}} \)=\(({\mathcal{\bm{X}}}_1, \dots, {\mathcal{\bm{X}}}_N) \)), and \( \lambda_i \) is a constant. and \( \|\cdot\|_{F} \) represents the Frobenius norm.   Assuming each \( \bm{\mathcal{X}}_i \) follows an isotropic distribution and \( \bm{\mathcal{X}}_1\)\dots\(\bm{\mathcal{X}}_N \) are mutually independent, we have:
\begin{equation}
\small
    \mathbb{E}_\mathcal{\bm{X}} [ \| \bm{W}_i^{T} \mathcal{\bm{X}}_i - \bm{W}^{T} \mathcal{\bm{X}}_i \|_{F}^2 ] = \frac{1}{D} \mathbb{E}_{\mathcal{\bm{X}}_i} [\| \mathcal{\bm{X}}_i \|_F^2 ] \| \bm{W}_i - \bm{W} \|_{F}^2
    \label{eq:linear_equ}
\end{equation}
where \( D \) is the dimension of each $\mathcal{\bm{X}}_i$. we have the following based on Eq. \ref{eq:linear_equ}:
\small{
    \begin{align}
    \bm{W}^{*} &= \mathop{\arg\min}_{\bm{W}} \mathbb{E}_{\mathcal{\bm{X}}} [\sum_{i=1}^N \lambda_i \| \bm{W}_i^{T} \mathcal{\bm{X}}_i - \bm{W}^{T} \mathcal{\bm{X}}_i \|_{F}^2 ] \\
    &= \mathop{\arg\min}_{\bm{W}} \sum_{i=1}^N \mathbb{E}_{\mathcal{\bm{X}}_i} [\lambda_i \| \bm{W}_i^{T} \mathcal{\bm{X}}_i - \bm{W}^{T} \mathcal{\bm{X}}_i \|_{F}^2 ] \\
    &= \mathop{\arg\min}_{\bm{W}} \sum_{i=1}^N \frac{\lambda_i}{D} \mathbb{E}_{\mathcal{\bm{X}}_i} \left[\| \mathcal{\bm{X}}_i \|_F^2 \right] \| \bm{W}_i - \bm{W} \|_{F}^2
\label{eq:linear_solution_process}
\end{align}
}
This expression admits a closed-form solution.
\begin{equation}
\bm{W}^{*}=\sum_{i=1}^N{\tilde{\lambda}_i\bm{W}_i},\tilde{\lambda}_i=\frac{\lambda _i \mathbb{E}_{\mathcal{\bm{X}}_i} [  \| \mathcal{\bm{X}}_i  \|_{F} ^2  ]}{\Sigma _{j=1}^{N}\lambda _j \mathbb{E}_{\mathcal{\bm{X}}_j} [  \| \mathcal{\bm{X}}_j  \|_{F} ^2  ]}
\label{eq:linear_solution_app}
\end{equation}

\subsection{Real-distribution-based Merging}
We can derive the following from the linear merging derivation in Subsection~\ref{sec:linear_merging_subsec}, and set each $\lambda_{i}$ to 1:
\begin{equation}
\small
    \bm{W}^{*} = \mathop{\arg\min}_{\bm{W}} \sum_{i=1}^{N} \mathbb{E}_{\bm{\mathcal{X}}_i} [ \| \bm{W}_i^{T} \bm{\mathcal{X}}_i - \bm{W}^{T} \bm{\mathcal{X}}_i \|_F^2 ].
    \label{eq:linear_independent}
\end{equation}
To compute each expectation in Eq.~\ref{eq:linear_independent}, we can sample from the distribution of \( \bm{\mathcal{X}}_i \), and using the law of large numbers, approximate the expectation as:  
\small{
    \begin{align}
    \mathbb{E}_{\bm{\mathcal{X}}_i} [ \| \bm{W}_i^{T} \bm{\mathcal{X}}_i - \bm{W}^{T} \bm{\mathcal{X}}_i \|_F^2 ] 
    &\approx \frac{1}{S} \sum_{s=1}^{S} \| \bm{W}_i^{T} \bm{x}_{is} - \bm{W}^{T} \bm{x}_{is} \|_F^2 \\
    &= \frac{1}{S} \| \bm{W}_i^{T} \bm{X}_i - \bm{W}^{T} \bm{X}_i \|_F^2
    \end{align}
}
where $\bm{x}_{is} \in \text{Sample}(\bm{\mathcal{X}}_i)$ and $\bm{X}_i = (\bm{x}_{i1}, \bm{x}_{i2}, \dots, \bm{x}_{iS})$. Therefore, we can reformulate the optimization objective based on the real distribution:
\begin{equation}
\small
    \bm{W}^{*} = \mathop{\arg\min}_{\bm{W}} \sum_{i=1}^{N} \| \bm{W}_i^{T} \bm{X}_i - \bm{W}^{T} \bm{X}_i \|_F^2.
\end{equation}
In fact, this optimization problem can be viewed as a linear regression problem, where $\bm{X}=[ \bm{X}_1,\bm{X}_2,\cdots ,\bm{X}_N ]^T$ is mapped to $\bm{Y}=[ \bm{W}_{1}^{T}\bm{X}_1,\bm{W}_{2}^{T}\bm{X}_2,\cdots ,\bm{W}_{N}^{T}\bm{X}_N ]^T$. Thus, the problem has a closed-form solution: 
\small{
    \begin{align}
\bm{W}^{*}&=( \bm{X}^T\bm{X} ) ^{-1}\bm{X}^T\bm{Y} \\
&=(\sum_{i=1}^N{\bm{X}_i\bm{X}_{i}^{T}})^{-1}(\sum_{i=1}^N{\bm{X}_i\bm{X}_{i}^{T}}\bm{W}_i)
\end{align}
}
Similarly, for the optimization problem corresponding to our algorithm in Eq. 5 of Section 3, we can also obtain its solution.
\subsection{Maximum Iteration Limit for IterIS}
Starting with the topology of the generative model, we construct the gradient computation graph \( G_{\nabla} \), which is a directed acyclic graph (DAG). To create the new graph \( G_M \), we extract all nodes corresponding to the input features for each LoRA. We follow a specific rule to construct \( G_M \): if there is a directed path from node \( A \) to node \( B \) in \( G_{\nabla} \), we establish a directed edge from \( A \) to \( B \) in \( G_M \). The resulting graph \( G_M \) is also a directed acyclic graph. We will demonstrate that \emph{the length of the longest directed path in \( G_M \), originating from any input node (of which there may be multiple), minus one, provides the maximum number of iterations required for the IterIS’s convergence.}

\noindent\textbf{Proof:} Let \( s \) denote the length of the longest path in \( G_M \) originating from the input node \( O_{\text{in}} \). We define a function \( g : v(G_M) \setminus \{O_{\text{in}}\} \rightarrow \{1, 2, \ldots, s\} \), where \( g(A) \) indicates the length of the longest path from \( O_{\text{in}} \) to node \( A \). We will use mathematical induction to demonstrate that at the \( k \)-th iteration, all nodes in \( g^{-1}(\{1, 2, \ldots, k+1\}) \) and their corresponding updated matrices remain unchanged in subsequent iterations. This observation relies on the fact that if the unified adapter's input \( \tilde{X}_i \) remains constant during iterations, the computed \( W_i \) will also remain constant.

\textbf{1. Base Case ( \( k = 0 \) ):}  
   For the initial iteration, it is clear that \( g^{-1}(1) \) is non-empty and contains only nodes with \( O_{\text{in}} \) as their sole parent. Therefore, \( g^{-1}(1) \) is entirely dependent on the input, indicating that these nodes and their corresponding matrices will remain unchanged in subsequent iterations.

\textbf{2. Inductive Step (Assume true for \( k = k_0 \)):}
   Assume that at iteration \( k = k_0 \), all nodes in \( g^{-1}(\{1, 2, \ldots, k_0 + 1\}) \) and their associated matrices remain constant. Since each node in \( g^{-1}(k_0 + 2) \) has its parent nodes contained within \( g^{-1}(\{1, 2, \ldots, k_0 + 1\}) \), it follows that the nodes in \( g^{-1}(k_0 + 2) \) are reliant on the unchanged nodes in \( g^{-1}(\{1, 2, \ldots, k_0 + 1\}) \). Consequently, these nodes and their corresponding updated matrices will also remain constant in subsequent iterations.

By this reasoning, when \( k = s - 1 \), it holds that \( g^{-1}(\{1, 2, \ldots, s\}) = v(G_M) \setminus \{O_{\text{in}}\} \) will remain unchanged in subsequent iterations. Thus, we prove and compute the upper bound on the maximum number of iterations required for the convergence of the IterIS algorithm.

For a transformer model consisting of \( L \) layers of encoders and \( L \) layers of decoders, if we apply LoRA fine-tuning to the \( k \) and \( v \) matrices within the attention modules, our algorithm will converge in no more than \( 3L - 1 \) iterations. As illustrated in Figure~\ref{fig:appendix_1}, the red-marked path has a length of 3, indicating that the algorithm converges after two iterations.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.478\textwidth]{pictures/supp-4.pdf} % 图
    \vspace{-2.2em}
    \caption{\textbf{Illustration of the maximum iteration count in graph \( G_M \).} For a transformer composed of one encoder and one decoder, the abstracted \( G_M \) after LoRA fine-tuning on the \( k \) and \( v \) matrices allows IterIS to converge within two iterations.}
    \label{fig:appendix_1}
\end{figure}

\begin{table}[t]
\centering
\fontsize{12}{13}\selectfont
\renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{5pt}  % Adjusted column spacing for better readability
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|cccccccc}
\toprule
         & \textbf{B-1} & \textbf{B-2} & \textbf{B-3} & \textbf{B-4} & \textbf{RougeL} & \textbf{CIDEr} & \textbf{ACC$_{POS}$} & \textbf{ACC$_{NEG}$} \\
\midrule
\textbf{LoRA$_{1}$} & 0.570 & 0.369 & 0.241 & 0.159 & 0.426 & 0.808 & 0.848 & 0.018 \\
\textbf{LoRA$_{2}$} & 0.550 & 0.354  & 0.234 & 0.157 & 0.414  & 0.811 & 0.138 & 0.867 \\
\bottomrule
\end{tabular}}
\vspace{-0.7em}
\caption{\textbf{Performance of style-specific LoRAs for multi-style caption on vision-language model.}}
\label{tab:performance_scores_vl}
\end{table}

\begin{table}[t]
\centering
\fontsize{8}{10}\selectfont
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{8pt} % Adjust column spacing for better readability
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
 \textbf{COLA} & \textbf{RTE} & \textbf{SST2} & \textbf{MNLI} & \textbf{QQP} & \textbf{QNLI} & \textbf{MRPC} \\
\midrule
 {0.532} & {0.812} & {0.946} & {0.855} & {0.858} & {0.920} & {0.831} \\
\bottomrule
\end{tabular}}
\vspace{-1em}
\caption{\textbf{Performance of task-specific LoRAs for multi-task integration on large language model.}}
\label{tab:performance_scores_multi}
\end{table}
\begin{table}[t]
\centering
\fontsize{8}{10}\selectfont  % Reduced font size for compactness
\renewcommand{\arraystretch}{1}  % Reduced row height for a tighter look
\setlength{\tabcolsep}{8pt}  % Slightly increased column spacing for readability
\begin{tabular}{cccc}
\toprule
 \textbf{TEC} & \textbf{Emoint} & \textbf{ISEAR} & \textbf{EC} \\
\midrule
 0.669 & 0.828 & 0.767 & 0.947 \\
\bottomrule
\end{tabular}
\vspace{-1em}
\caption{\textbf{Performance of task-specific LoRAs for in-domain task integration on large language model.}}
\label{tab:performance_scores_indomain}
\end{table}

\section{Detailed Experimental Setting}
\label{sec:B}
\subsection{Datasets}

\noindent\textbf{DreamBooth~\cite{ruiz2023dreambooth}}. 
The DreamBooth dataset consists of 30 subjects across 15 different classes. Among these, 9 are live subjects (dogs and cats), while the remaining 21 are objects. Each subject is represented by a variable number of images (ranging from 4 to 6), typically captured under diverse conditions, in various environments, and from different angles.

\noindent\textbf{Customconcept101~\cite{kumari2023multi}}. 
The customconcept101 dataset, introduced by custom diffusion~\cite{kumari2023multi}, comprises 101 concepts, each represented by 3 to 15 images, designed to evaluate model customization methods. 

\noindent\textbf{SentiCap}~\cite{mathews2016senticap}. The SentiCap dataset comprises thousands of images with sentiment-labeled captions. The POS subset includes 2,873 positive sentences paired with 998 images for training and 2,019 sentences paired with 673 images for testing. The NEG subset contains 2,468 negative sentences with 997 images for training and 1,509 sentences with 503 images for testing.

\noindent\textbf{GLUE}~\cite{wang2018glue}. The GLUE dataset serves as a benchmark for evaluating natural language understanding models. It encompasses multiple tasks, including sentiment analysis, textual entailment, and sentence similarity. For our evaluation, we utilize the SST-2~\cite{socher2013recursive}, MRPC~\cite{dolan2005automatically}, MNLI~\cite{williams2017broad}, QNLI~\cite{rajpurkar2016squad},  RTE~\cite{giampiccolo2007third}, COLA~\cite{warstadt2019cola}, and QQP  datasets. Evaluations are conducted on the official development sets, as the test labels remain hidden.

\noindent\textbf{Emotion}. For emotion classification, we use the preprocessed datasets provided by Oberlander \& Klinger ~\cite{bostan2018analysis}, specifically TEC~\cite{mohammad2012emotional}, ISEAR~\cite{scherer1994evidence}, Emoint~\cite{mohammad2017wassa}, and Emotion-Cause (EC)~\cite{ghazi2015detecting}, for domain-specific training. All four datasets include the emotion classes of anger, fear, joy, and sadness in their label space, encompassing various scenarios and sources. In our experiments, each dataset is randomly divided into training and testing sets, with five parts for training and one part for testing.

\noindent\textbf{FlickrStyle10K~\cite{gan2017stylenet}}. 
The FlickrStyle10K dataset is derived from the Flickr30K~\cite{plummer2015flickr30k} image caption dataset. It originally contained 10,000 image-caption pairs with stylized captions in humorous and romantic styles. However, only 7,000 pairs from the official training set are currently publicly available.

% \subsection{Evaluation Metrics}
% In the image captioning task, we evaluate text generation quality using BLEU-1 to BLEU-4~\cite{papineni2002bleu}, ROUGE-L\cite{lin2004rouge}, and CIDER~\cite{vedantam2015cider}, while employing accuracy (ACC) to assess whether the model can correctly generate captions in the specified style. We utilized SentiWordNet~\cite{sebastiani2006sentiwordnet} as the caption style classifier for SentiCap datasets. Within the GLUE benchmark, all tasks utilize ACC for performance measurement, except for CoLA, which uses the Matthews correlation coefficient (MCC)~\cite{matthews1975comparison}. For the emotion classification task, we assess all four emotion datasets using the Macro-F1 score.
% All prompts used in our experiments are provided in the Appendix.
\begin{table*}[t]
\centering
% \scriptsize  % Smaller font size for better fit in the double-column format
\fontsize{8.1}{10}\selectfont
\renewcommand{\arraystretch}{1}  % Adjusted row height for better spacing
\setlength{\tabcolsep}{5pt}  % Adjust column spacing for better readability
\begin{tabular}{c|ccccccccccccccc}
\toprule
\textbf{Iteration} & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 \\
\midrule
\textbf{ACC$_{mean}$} & 0.674 & 0.919 & 0.681 & 0.862 & 0.729 & 0.806 & 0.789 & 0.788 & 0.786 & 0.784 & 0.784 & 0.784 & 0.784 & 0.784 & 0.784 \\
\midrule
\textbf{CIDEr$_{mean}$} & 0.785 & 0.381 & 0.793 & 0.651 & 0.798 & 0.794 & 0.791 & 0.770 & 0.789 & 0.790 & 0.791 & 0.790 & 0.790 & 0.790 & 0.790 \\
\midrule
\textbf{Score$_{aver}$} & 0.730 & 0.650 & 0.737 & 0.756 & 0.764 & 0.800 & 0.790 & 0.779 & 0.788 & 0.787 & 0.788 & 0.787 & 0.787 & 0.787 & 0.787 \\
\bottomrule
\end{tabular}
\vspace{-0.8em}
\caption{\textbf{Performance across different maximum iterations.}}
\vspace{-1.2em}
\label{tab:iteration_scores}
\end{table*}

\subsection{LoRA Training}
\noindent\textbf{LoRAs for Multi-concept Customization}. 
We applied the widely-used DreamBooth-LoRA~\cite{ruiz2023dreambooth} tuning to generate multiple LoRAs for stable diffusion v1.5~\cite{rombach2022high}, with each LoRA dedicated to a single new concept. The LoRA rank was set to 32, and LoRA alpha was set to 1. During the textual inversion phase, we used a learning rate of \( 5 \times 10^{-4} \), with each new concept represented by a single learnable token, all initialized uniformly. In the subsequent fine-tuning phase, the UNet and text encoder were trained with learning rates of \( 10^{-4} \) and \( 10^{-5} \), respectively, while the textual inversion learning rate was maintained at \( 10^{-4} \).  Both phases involved training for 800 steps, with a batch size of 1 and gradient accumulation steps set to 4.

\noindent\textbf{LoRAs for Multi-style Caption}. 
We applied LoRA tuning to fine-tune the BLIP-image-caption-base~\cite{li2022blip}. LoRAs were integrated into all self-attention modules within the text encoder, specifically targeting the \(q\), \(v\), and \(k\) matrices~\cite{vaswani2017attention}. The LoRA rank was set to 32, with \(\alpha\) set to 32, and a dropout rate of 0.05. The training was conducted with a batch size of 8 for a maximum of 15 epochs, using an initial learning rate of 3e-5. The AdamW~\cite{kingma2014adam} optimizer was employed for optimization. Table~\ref{tab:performance_scores_vl} summarizes the key metrics of multiple LoRAs trained in this part.
% \hspace*{1.2em}\textbf{Pre-trained Models}.
% In the same set of experiments, all agents share an identical architecture, which stems from LoRA fine-tuning of a common pre-trained model. For the multi-style image captioning task, we utilize the classic BLIP-image-caption-base~\cite{li2022blip} model as the foundational pre-trained model. For the multi-task experiments on the GLUE dataset, we employ two distinct pre-trained encoder-decoder models: Flan-T5-base~\cite{https://doi.org/10.48550/arxiv.2210.11416} and BART~\cite{lewis2019bart}. However, during the LoRA fine-tuning of BART on the RTE dataset, we observe that BART struggles to perform effectively in this task. Consequently, we do not evaluate our method using BART for the RTE dataset. In the emotion classification experiments, we leverage the state-of-the-art Flan-T5-large~\cite{https://doi.org/10.48550/arxiv.2210.11416} as our pre-trained model.

% \textbf{LoRA Training}.
% In our experiments, LoRA fine-tuning is applied exclusively to the Query, Key, and Value~\cite{vaswani2017attention} matrices of the attention modules, with LoRA alpha values consistently set to 32.0. During training, we utilize the Adam optimizer. For the multi-style image captioning task, the rank for fine-tuning BLIP is set to 32, while all other tasks employ a rank of 8. Further details on the LoRA training configurations are provided in the Appendix.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.478\textwidth]{pictures/supp-3.pdf} % 图
    \vspace{-2em}
    \caption{\textbf{Performance across different maximum iterations}}
    \label{fig:appendix_2}
    \vspace{-1em}
\end{figure}

\noindent\textbf{LoRAs for Multiple NLP tasks Integration.} \textbf{1)} In-domain task integration: We fine-tuned FLAN-t5-large~\cite{https://doi.org/10.48550/arxiv.2210.11416} using LoRA tuning, targeting the \(q\) and \(v\) matrices of all attention layers ~\cite{vaswani2017attention}. The learning rate was set to 5e-5, with a training duration of 10 epochs and a batch size of 12. A warm-up phase \cite{he2016deep} of 100 steps was applied. Optimization was performed using the AdamW optimizer~\cite{kingma2014adam}, with a weight decay of 0.001. \textbf{2)} Multi-task integration: We fine-tuned FLAN-T5-base~\cite{https://doi.org/10.48550/arxiv.2210.11416} using LoRA on the \(q\) and \(v\) matrices across all attention layers~\cite{vaswani2017attention}. The learning rate was set to either \(5 \times 10^{-5}\) or \(1 \times 10^{-5}\), with training durations of 8 or 10 epochs and batch sizes of 12 or 16. A 100-step warm-up phase~\cite{he2016deep} was applied.   
The AdamW optimizer~\cite{kingma2014adam} was used with a weight decay of 0.001. For further detailed training configurations for each subset, please refer to the forthcoming release of our code. 
Table~\ref{tab:performance_scores_multi} and Table~\ref{tab:performance_scores_indomain} summarize the key metrics of the LoRAs trained in this part.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{pictures/supp-1.pdf} % 图
    \vspace{-2em}
    \caption{\textbf{Additional qualitative results for multi-concept customization.} Target images represent individual concepts used in the compositions. (a) Examples of pairwise compositions generated by our method. (b) Examples of individual concepts generated by IterIS.}
    \label{fig:appendix_4}
\end{figure*}

\subsection{Baseline Training Details}
\noindent\textbf{Textual Inversion~\cite{gal2022image}.} We employed uniformly initialized learnable tokens with a batch size of 1 and set the gradient accumulation steps to 4. The learning rate was configured to \( 5 \times 10^{-4} \), and the training was carried out over a total of 800 steps. Each new concept was represented as ``[adj\_n] n,'' where ``[adj\_n]'' denoted a learnable token. For instance, when introducing the new concept ``cat,'' we represented the new concept as ``[adj\_cat] cat''.

\noindent\textbf{Custom Diffusion~\cite{kumari2023multi}.} We utilized the official implementation of custom diffusion. To ensure a fair comparison, we adopted its optimization method as the baseline. The number of DDPM steps was set to 200, and the unconditional guidance scale was set to 6.

\noindent\textbf{Linear Merging~\cite{zhang2023composing}.} We performed linear merging using LoRAs with identical weights (e.g., average merging).

\noindent\textbf{RegMean~\cite{jin2022dataless}.} We utilized the official implementation of RegMean, with modifications to the interface. In our experiments, we reproduced RegMean by adopting its official regularization settings, with the regularization coefficient \(\alpha\) set to 0.1. Following the recommendations in the original paper, we set the number of inference samples to 100–200, with a batch size of 16. In cases where the dataset contained fewer than the recommended number, we used all available data. All other hyperparameters and LoRAs were kept consistent with those in our method.
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{pictures/supp-2.pdf} % 图
    \vspace{-1.5em}
    \caption{\textbf{More examples of style caption generated by our algorithm.}}
    \label{fig:appendix_3}
\end{figure*}

\section{Ablation Study of IterIS}
\label{sec:C}
\noindent\textbf{Influence on Maximum Iteration.} As shown in Figure~\ref{fig:appendix_2} and Table~\ref{tab:iteration_scores}, we evaluated the impact of varying maximum iterations in IterIS on vision-language model. Mean ACC, CIDEr, and score$_{aver}$ (defined as (ACC$_{mean}$ + CIDEr$_{mean}$) / 2) were computed on the validation sets of the POS and NEG datasets. When limited to 4 or fewer iterations, IterIS exhibits notable instability, starting with a low score$_{aver}$ that progressively improves. Peak performance is observed at 5 iterations, beyond which a slight decline suggests potential overfitting. Performance stabilizes after 11 iterations, aligning with our theoretical expectations.
\begin{table}[t]
\centering
\fontsize{9}{10}\selectfont
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{4pt} % Adjust column spacing
\resizebox{\columnwidth}{!}{ % Ensure table fits within the column width
\begin{tabular}{l|cccccc}
\toprule
    & B-1   & B-2   & B-3   & B-4   & Rough-L & CIDEr \\ \midrule
POS (Ours w/o Reg)  & 0.480 & 0.291 & 0.180 & 0.112 & 0.368   & 0.534 \\
POS (Ours w/ Reg)    & \textbf{0.561} & \textbf{0.359} & \textbf{0.232} & \textbf{0.151} & \textbf{0.420}   & \textbf{0.794} \\
 \midrule
NEG (Ours w/o Reg)  & 0.356 & 0.206 & 0.127 & 0.079 & 0.334   & 0.476 \\ 
NEG (Ours w/ Reg)    & \textbf{0.540} & \textbf{0.348} & \textbf{0.230} & \textbf{0.153} & \textbf{0.406}   & \textbf{0.794} \\
\bottomrule
\end{tabular}}
\caption{\textbf{Performance comparison of our algorithm with and without the regularization term for vision-language model}. The \textbf{bold} numbers highlight the best performance.}
\label{tab:Regularization}
\end{table}

\begin{table}[t] 
\centering
\fontsize{8}{9}\selectfont
\renewcommand{\arraystretch}{1}  % 调整行间距，使表格更易读
\setlength{\tabcolsep}{3pt}        % 调整列间距，使表格更加紧凑
\begin{tabular}{l|ccc}
\toprule
Composition & \textbf{(MRPC, SST2)} & \textbf{(COLA, MNLI)} & \textbf{(RTE, MRPC)} \\ \midrule
Ours w/o Reg & (0.272, 0.177) & (0.0, 0.0) &  (0.671, 0.667)\\
Ours w/ Reg & \textbf{(0.824, 0.951)} & \textbf{(0.299, 0.780)} &\textbf{(0.805, 0.814)} \\
\bottomrule
\end{tabular}

\caption{\textbf{Performance comparison of our algorithm with and without the regularization term for LLM.} The first dataset pair consists of MRPC and SST2, and so on. The \textbf{bold} numbers indicate the best performance within each dataset pair.}
\label{tab:regularization_comparison}
\end{table}

\begin{table}[t]
\centering
\fontsize{8}{9}\selectfont  % Adjusted font size for readability
\renewcommand{\arraystretch}{1.1}  % Adjusted row height for better spacing
\setlength{\tabcolsep}{3pt}  % Adjusted column spacing for better readability
\begin{tabular}{l|ccc}
\toprule
  Composition      & \textbf{(COLA, MNLI)}   & \textbf{(MNLI, SST2)} & \textbf{(COLA, SST2)}  \\
\midrule
Ours w/o Weights & (0.271, 0.728)          & (0.761, 0.945)   & (0.356, 0.943)       \\
Ours w/ Weights   & \textbf{(0.299, 0.780)}          & \textbf{(0.764, 0.945)}    & \textbf{(0.360, 0.943)}       \\
\bottomrule
\end{tabular}
\caption{\textbf{Performance comparison of our algorithm with and without adaptive weights for LLM.} The first dataset pair consists of COLA and MNLI, and so on. The \textbf{bold} numbers indicate the best performance within each dataset pair.}
\label{tab:coef_performance}
\vspace{-2em}
\end{table}

\noindent\textbf{Influence on Regularization Term.}
Using 50 samples for inference, we evaluated the effect of the introduced regularization term on the performance of IterIS for both the vision-language model and the large language model. As demonstrated in Table~\ref{tab:Regularization} and Table~\ref{tab:regularization_comparison}, incorporating the regularization term results in substantial performance improvements, highlighting its pivotal role in enhancing the effectiveness of IterIS.

\noindent\textbf{Influence on Adaptive Weights.}
We assessed the impact of adaptive weights on algorithm performance, as summarized in Table~\ref{tab:coef_performance}. The results demonstrate that adaptive weights can enhance algorithm performance to a certain extent. Moreover, we observe that when there are greater discrepancies between different tasks, the application of our proposed adaptive weights leads to a more noticeable improvement (\eg, COLA and MNLI).

\begin{table}[t]
\centering
\fontsize{7}{8}\selectfont
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{5pt} % 调整垂直间距
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l|cccccc}
\toprule
\textbf{Style}       & \textbf{Method} & \textbf{B-1} & \textbf{B-2} & \textbf{B-3} & \textbf{B-4} & \textbf{Cider} & \textbf{ACC} \\ \midrule
\multirow{3}{*}{\textbf{POS}} 
                     & RegMean         & 0.576 & 0.368 & 0.239 & 0.156 & \textbf{0.801} & 0.624 \\
                     & Linear          & 0.561 & 0.357 & 0.230 & 0.151 & 0.771 & 0.522 \\ 
                     & IterIS          & 0.561 & 0.359 & 0.232 & 0.151 & 0.794 & \textbf{0.830} \\ \midrule
\multirow{3}{*}{\textbf{NEG}} 
                     & RegMean         & 0.540 & 0.341 & 0.223 & 0.144 & 0.779 & 0.692 \\
                     & Linear          & 0.509 & 0.319 & 0.206 & 0.133 & 0.733 & 0.557 \\
                     & IterIS          & 0.540 & 0.348 & 0.230 & 0.153 & \textbf{0.794} & \textbf{0.781} \\ \midrule
\multirow{3}{*}{\textbf{HUM}} 
                     & RegMean         & 0.303 & 0.174 & 0.103 & 0.061 & 0.528 & -\\
                     & Linear          & 0.281 & 0.161 & 0.095 & 0.055 & 0.504 & -\\ 
                    & IterIS          & 0.300 & 0.174 & 0.103 & 0.060 & \textbf{0.530} & -\\ \midrule
\multirow{3}{*}{\textbf{ROM}} 
                     & RegMean         & 0.307 & 0.172 & 0.101 & 0.061 & 0.523 & -\\
                     & Linear          & 0.266 & 0.151 & 0.054 & 0.047 & 0.487 & -\\ 
                     & IterIS          & 0.308 & 0.172 & 0.101 & 0.062 & \textbf{0.524} & -\\ \bottomrule
\end{tabular}%
}
\caption{\textbf{Detailed performance comparison for multi-style caption generation} includes two combinations: \textbf{(1)} ``positive'' (POS) + ``negative'' (NEG), and \textbf{(2)} ``humor'' (HUM) + ``romance'' (ROM). The \textbf{bold} values highlight the best performance. }
\label{tab:style_metrics}
\vspace{-1.5em}
\end{table}

\section{More Results}
\label{sec:D}
\noindent\textbf{More Results on Text-to-Image Diffusion.}
Figure~\ref{fig:appendix_4}(a) showcases additional combinations of pairwise concepts from our experiments, while Figure~\ref{fig:appendix_4}(b) illustrates the individual concepts generated by the composed LoRAs. Our method exhibits robust performance across a wide range of multi-concept combinations.   
\begin{table*}[t]
\centering
\fontsize{8.1}{10}\selectfont
\renewcommand{\arraystretch}{1.2} % Adjust row spacing
\setlength{\tabcolsep}{3pt} % Adjust column spacing
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
                     & \multicolumn{3}{c|}{\textbf{Score$_1$}}      & \multicolumn{3}{c|}{\textbf{Score$_2$}}      & \multicolumn{3}{c|}{\textbf{Score$_3$}}      & \multicolumn{3}{c}{\textbf{Score$_4$}}      \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
\textbf{Composition}     & \textbf{IterIS} & \textbf{RegMean} & \textbf{Linear} & \textbf{IterIS} & \textbf{RegMean} & \textbf{Linear} & \textbf{IterIS} & \textbf{RegMean} & \textbf{Linear} & \textbf{IterIS} & \textbf{RegMean} & \textbf{Linear} \\ 
\midrule
Emoint/EC            & \textbf{{0.810}} & 0.808 & 0.784 & \textbf{{0.938}} & 0.922 & 0.912 & -     & -     & -     & -     & -     & -     \\
Emoint/TEC           & \textbf{{0.807}} & 0.758 & 0.731 & \textbf{{0.551}} & 0.544 & 0.474 & -     & -     & -     & -     & -     & -     \\
Emoint/ISEAR         & \textbf{{0.811}} & 0.786 & 0.733 & \textbf{{0.665}} & 0.650 & 0.603 & -     & -     & -     & -     & -     & -     \\
EC/TEC               & \textbf{{0.945}} & 0.926 & 0.881 & 0.603 & \textbf{{0.630}} & 0.592 & -     & -     & -     & -     & -     & -     \\
EC/ISEAR             & \textbf{{0.953}} & 0.938 & 0.900 & 0.709 & \textbf{{0.719}} & 0.679 & -     & -     & -     & -     & -     & -     \\
TEC/ISEAR            & 0.574 & \textbf{{0.592}} & 0.526 & \textbf{{0.710}} & 0.661 & 0.631 & -     & -     & -     & -     & -     & -     \\
Emoint/EC/TEC        & \textbf{{0.782}} & 0.753 & 0.727 & \textbf{{0.942}} & 0.923 & 0.877 & \textbf{{0.540}} & 0.510 & 0.460 & -     & -     & -     \\
Emoint/EC/ISEAR      & \textbf{{0.795}} & 0.774 & 0.720 & \textbf{{0.935}} & 0.926 & 0.887 & \textbf{{0.670}} & 0.641 & 0.593 & -     & -     & -     \\
Emoint/TEC/ISEAR     & \textbf{{0.786}} & 0.721 & 0.683 & \textbf{{0.500}} & 0.499 & 0.455 & \textbf{{0.646}} & 0.607 & 0.593 & -     & -     & -     \\
EC/TEC/ISEAR         & \textbf{{0.950}} & 0.910 & 0.857 & 0.552 & \textbf{{0.555}} & 0.486 & \textbf{{0.683}} & 0.649 & 0.614 & -     & -     & -     \\
Emoint/EC/TEC/ISEAR  & \textbf{{0.776}} & 0.714 & 0.688 & \textbf{{0.935}} & 0.901 & 0.873 & \textbf{{0.508}} & 0.481 & 0.445 & \textbf{{0.657}} & 0.607 & 0.590 \\
\bottomrule
\end{tabular}
\caption{\textbf{Performance of all possible compositions in in-domain task integration.} Score$_i$ denotes the performance metric for the i-th task within the composition. The \textbf{bold} values highlight the best performance.}
\label{tab:results_indomain_task}
\end{table*}
\begin{table}[t]
\centering
\fontsize{8.1}{10}\selectfont
\renewcommand{\arraystretch}{1.2} % Adjust row spacing
\setlength{\tabcolsep}{2pt} % Adjust column spacing
\begin{tabular}{l|ccc|ccc}
\toprule
                           & \multicolumn{3}{c|}{\textbf{Score$_1$}}                                                          & \multicolumn{3}{c}{\textbf{Score$_2$}}                                                          \\ \midrule
\textbf{Composition} & \textbf{IterIS}                & \textbf{RegMean}             & \textbf{Linear}              & \textbf{IterIS}                & \textbf{RegMean}             & \textbf{Linear}              \\ \midrule
MNLI/RTE                   & { \textbf{0.831}} & 0.803                        & 0.751                        & { \textbf{0.794}} & 0.787                        & 0.776                        \\
MNLI/COLA                  & { \textbf{0.780}} & 0.755                        & 0.765                        & 0.299                        & 0.279                        & { \textbf{0.383}} \\
MNLI/SST2                  & { \textbf{0.764}} & 0.747                        & 0.645                        & { \textbf{0.945}} & { \textbf{0.945}} & 0.942                        \\
MNLI/QQP                   & { \textbf{0.821}} & 0.813                        & 0.687                        & { \textbf{0.855}} & 0.853                        & 0.842                        \\
MNLI/QNLI                  & { \textbf{0.821}} & 0.806                        & 0.797                        & { \textbf{0.916}} & 0.914                        & 0.905                        \\
MNLI/MRPC                  & { \textbf{0.825}} & 0.816                        & 0.744                        & { \textbf{0.821}} & 0.792                        & 0.772                        \\
RTE/COLA                   & { \textbf{0.787}} & 0.783                        & 0.733                        & 0.311                        & 0.307                        & { \textbf{0.388}} \\
RTE/SST2                   & { \textbf{0.819}} & 0.809                        & 0.773                        & 0.946                        & { \textbf{0.948}} & 0.943                        \\
RTE/QQP                    & 0.816                        & 0.812                        & { \textbf{0.819}} & 0.856                        & { \textbf{0.856}} & 0.853                        \\
RTE/QNLI                   & 0.805                        & 0.805                        & { \textbf{0.812}} & 0.919                        & { \textbf{0.920}} & 0.913                        \\
RTE/MRPC                   & 0.805                        & { \textbf{0.812}} & 0.805                        & { \textbf{0.814}} & 0.801                        & 0.757                        \\
COLA/SST2                  & { \textbf{0.360}} & 0.291                        & 0.233                        & { \textbf{0.943}} & 0.938                        & 0.891                        \\
COLA/QQP                   & 0.386                        & 0.332                        & { \textbf{0.397}} & { \textbf{0.839}} & 0.831                        & 0.734                        \\
COLA/QNLI                  & 0.297                        & 0.305                        & { \textbf{0.346}} & { \textbf{0.906}} & 0.904                        & 0.818                        \\
COLA/MRPC                  & 0.341                        & 0.307                        & { \textbf{0.383}} & 0.811                        & { \textbf{0.816}} & 0.765                        \\
SST2/QQP                   & { \textbf{0.947}} & { \textbf{0.947}} & 0.936                        & { \textbf{0.855}} & 0.854                        & 0.839                        \\
SST2/QNLI                  & { \textbf{0.943}} & { \textbf{0.943}} & { \textbf{0.943}} & { \textbf{0.920}} & 0.916                        & 0.882                        \\
SST2/MRPC                  & { \textbf{0.951}} & 0.947                        & 0.939                        & { \textbf{0.824}} & 0.809                        & 0.794                        \\
QQP/QNLI                   & { \textbf{0.856}} & 0.856                        & 0.846                        & { \textbf{0.920}} & 0.920                        & 0.915                        \\
QQP/MRPC                   & { \textbf{0.855}} & 0.854                        & 0.846                        & { \textbf{0.816}} & 0.814                        & 0.801                        \\
QNLI/MRPC                  & { \textbf{0.922}} & 0.920                        & 0.907                        & { \textbf{0.821}} & { \textbf{0.821}} & 0.797                        \\ \bottomrule
\end{tabular}
\caption{\textbf{Performance of all pairwise compositions in multi-task integration.} Score$_i$ denotes the performance metric for the i-th task within the composition. The \textbf{bold} values highlight the best performance.}
\vspace{-1em}
\label{tab:results_multi_task}
\end{table}

\begin{table}[t] 
\centering
\fontsize{8}{9}\selectfont
\renewcommand{\arraystretch}{1}  % 调整行间距，使表格更易读
\setlength{\tabcolsep}{3pt}        % 调整列间距，使表格更加紧凑
\begin{tabular}{l|ccc}
\toprule
\textbf{Composition} & \textbf{(MRPC, SST2)} & \textbf{(SST2, QQP)} & \textbf{(QQP, MRPC)} \\ \midrule
\textbf{Task arithmetic} & (0.806, 0.937) & (0.937, 0.841) &  (0.845, 0.811)\\
\textbf{Ties merging} & (0.765, 0.943) & (0.944, 0.823) &(0.846, 0.806) \\
\textbf{Hyper-linear} & (0.809, 0.933) & (0.931, 0.849) &(0.846, 0.801) \\
\textbf{IterIS (Ours)} & \textbf{(0.824, 0.951)} & \textbf{(0.947,  0.855)} &\textbf{(0.855, 0.816)} \\
\bottomrule
\end{tabular}
\vspace{-1.1em}
\caption{\textbf{Performance for multi-task integration for additional three baselines.}}
\label{tab:NLP_comparison}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.478\textwidth]{pictures/supp-5.pdf} % 图
    \vspace{-2em}
    \caption{\textbf{The workflow diagram of our algorithm.}}
    \label{fig:appendix_5}
    \vspace{-1em}
\end{figure}
\noindent\textbf{More Results on V\&L Model.} 
As shown in Figure 6 of Section 4, we provide additional examples of positive and negative captions generated by our algorithm. A detailed version of Table 2 of Section 4 from the main text is presented in Table~\ref{tab:style_metrics}. Additionally, we conducted experiments on FlickrStyle10K~\cite{gan2017stylenet}, exploring combinations of two other distinct styles. The results are also included in Table~\ref{tab:style_metrics}. Due to the subjective nature of evaluating humor and romance, as well as the lack of the open test set, we didn't quantify humor(romance)-specific metrics. As a result, aside from the CIDEr score, the advantages of our algorithm for this style combination are less evident. 

\noindent\textbf{More Results on LLM.} 
A detailed version of Table 3 in Section, as discussed in the main text, is provided for reference in this part. Table~\ref{tab:results_indomain_task} summarizes the experimental results of 11 combinations for in-domain task integration, while Table~\ref{tab:results_multi_task} presents the results of 21 combinations for multi-task integration. Our proposed method outperforms both RegMean and linear merging in the majority of cases, highlighting its robustness and effectiveness. Additionally, Table~\ref{tab:NLP_comparison} shows the superiority of our method compared to three extra baselines in the multi-task integration subset.

\section{Others}
\label{sec:E}
\noindent\textbf{Illustration of IterIS.} To facilitate a better understanding of IterIS, we present Figure~\ref{fig:appendix_5}, which effectively illustrates the layer-wise characteristics and inference-solving process of our method.

\noindent\textbf{Efficiency Analysis.} IterIS ensures computation and memory efficiency through sample efficiency and limited iterations. In the V\&L experiments, we utilized 50 prompt-image pairs as inference samples and performed 6 iterations. For each layer, the total computational cost for computing a single inner product matrix is \( 50 \text{ (sample)} \times 6 \text{ (iteration)} = 300 \) one-dimensional tensor inner products. However, that cost for RegMean is \( 1600 \times 1 = 1600 \), which is much higher than IterIS. Moreover, sample efficiency of IterIS allows us to perform all computations without batching, ensuring memory efficiency. Notably, all experiments for IterIS were conducted using a single RTX 3090 GPU.

\noindent\textbf{Detailed Analysis for the Regularization Term and Adaptive Weights.} \textbf{1)} The regularization term prevents irreversible situations in solutions, which often occur in few-sample cases. In such cases, at least one solution to the optimization objective in Eq.(5) renders it zero. This means the output features in each layer of the merged model are equal to those in the corresponding layer of each individual model. Due to the limited number of inference samples, the risk of overfitting to these samples is high. Notably, we can infer that the optimal solution to Eq.(1) is close to the linear solution based on Eq.(2). Applying identity matrices as regularization terms aligns the solution more closely with the linear solution, enhancing robustness. However, diagonal matrices in RegMean cannot achieve the same effect. \textbf{2)} From a dimensional analysis perspective, the scale of the adaptive weights corresponds to that of $\|\bm{X}_{i}\|_F^{-2}$. This neutralizes the scale of $\bm{X}_{i}$ in the optimization objective ($\|\bm{W}_{i}^{T}\bm{X}_{i} - \bm{W}^{T}\tilde{\bm{X}}_{i}  \|_{F}^{2}$), thereby ensuring that the optimization objective remains unbiased to the scale of $\bm{X}_{i}$.

\noindent\textbf{Limitations.} Similar to other LoRA merging methods, performance degradation on individual tasks is inevitable when merging tasks of different types. This degradation becomes more pronounced as the diversity of task types increases or when parameter conflicts arise. Furthermore, since our method does not include domain-specific enhancements for text-to-image diffusion, it shares a limitation with custom diffusion—namely, the confusion of object concepts.
% \subsection{Limitations} Similar to other LoRA merging methods, when the tasks being merged involve different types, performance degradation on individual tasks is unavoidable. This degradation becomes more pronounced as the number of task types increases or in the presence of parameter conflicts. Additionally, since our method does not incorporate additional enhancements in the text-to-image diffusion domain, it faces the same issue as custom diffusion, namely, the confusion of object concepts. Examples of such cases are provided in the appendix. 
% \label{sec:rationale}
% % 
% Having the supplementary compiled together with the main paper means that:
% % 
% \begin{itemize}
% \item The supplementary can back-reference sections of the main paper, for example, we can refer to \cref{sec:intro};
% \item The main paper can forward reference sub-sections within the supplementary explicitly (e.g. referring to a particular experiment); 
% \item When submitted to arXiv, the supplementary will already included at the end of the paper.
% \end{itemize}
% % 
% To split the supplementary pages from the main paper, you can use \href{https://support.apple.com/en-ca/guide/preview/prvw11793/mac#:~:text=Delete%20a%20page%20from%20a,or%20choose%20Edit%20%3E%20Delete).}{Preview (on macOS)}, \href{https://www.adobe.com/acrobat/how-to/delete-pages-from-pdf.html#:~:text=Choose%20%E2%80%9CTools%E2%80%9D%20%3E%20%E2%80%9COrganize,or%20pages%20from%20the%20file.}{Adobe Acrobat} (on all OSs), as well as \href{https://superuser.com/questions/517986/is-it-possible-to-delete-some-pages-of-a-pdf-document}{command line tools}.

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

